Open-Access Full-Duplex Wireless in the ORBIT Testbed

In order to support experimentation with full-duplex (FD) wireless, we recently integrated an open-access FD transceiver in the ORBIT testbed. In this report, we present the design and implementation of the FD transceiver and interfaces, and provide examples and guidelines for experimentation. In particular, an ORBIT node with a National Instruments (NI)/Ettus Research Universal Software Radio Peripheral (USRP) N210 software-defined radio (SDR) was equipped with the Columbia FlexICoN Gen-1 customized RF self-interference (SI) canceller box. The RF canceller box includes an RF SI canceller that is implemented using discrete components on a printed circuit board (PCB) and achieves 40dB RF SI cancellation across 5MHz bandwidth. We provide an FD transceiver baseline program and present two example FD experiments where 90dB and 85dB overall SI cancellation is achieved for a simple waveform and PSK modulated signals across both the RF and digital domains. We also discuss potential FD wireless experiments that can be conducted based on the implemented open-access FD transceiver and baseline program.

==> tex/canceller.tex <==

%%
\begin{figure}[t]
\centering
\subfloat{
\label{fig:diagram-orbit-node}
\includegraphics[width=0.9\columnwidth]{figs/diagram_orbit_node.png}}
\vspace{-0\baselineskip}
\caption{Diagram of the implemented FD radio.}
\label{fig:diagram-orbit-node}
\vspace{-\baselineskip}
\end{figure}
%%

%%
\begin{figure}[t]
\centering
\subfloat{
\label{fig:canc-orbit-node}
\includegraphics[width=0.47\columnwidth]{figs/gen1_canc_box.png}}
\subfloat{
\label{fig:canc-orbit-node}
\includegraphics[width=0.5\columnwidth]{figs/gen1_orbit_node.png}}
\vspace{-0\baselineskip}
\caption{The Columbia FlexICoN Gen-1 RF SI canceller and the FD node installed in the ORBIT testbed.}
\label{fig:canc-orbit-node}
\vspace{-\baselineskip}
\end{figure}
%%

In this section, we describe the design and implementation of the conventional amplitude- and phase-based RF SI canceller, which is an improved version of that presented in~\cite{fd_demo_mobihoc16}.

%%
\subsection{The RF Canceller PCB}

To achieve SIC in the RF domain, the RF canceller taps a reference signal from the output of the power amplifier (PA) at the TX side and adjusts its amplitude and phase, and then performs SIC at the input of the low-noise amplifier (LNA) at the RX side. The implemented RF canceller PCB is optimized around $\SI{900}{MHz}$ operating frequency.\footnote{In this implementation, we select $\SI{900}{MHz}$ operating frequency but this approach can be easily extended to other frequencies (e.g., $2.4/\SI{5}{GHz}$).} For amplitude adjustment, a $7$-bit SKY12343-364LF digital attenuator is used, in which the attenuation can be adjusted within a $\SI{31.75}{dB}$ range at $\SI{0.25}{dB}$ step size. For phase adjustment, a passive phase-shifter is used, which covers full $\SI{360}{deg}$ with a resolution of $\SI{0.5}{deg}$, and is controlled by an $8$-bit TI-DAC081S101 digital-to-analog converter (DAC). Both the attenuator and the phase shifter are programmed via a serial-to-parallel interface (SPI), with code values represented by \texttt{ATT} (\underline{ATT}uation) and \texttt{PS} (\underline{P}hase \underline{S}hift), respectively, with tuning range
%%
\begin{align}
\texttt{ATT} \in \{0,1,\cdots,127\},\ \texttt{PS} \in \{0,1,\cdots,255\}. \nonumber
\end{align}
%%
Fig.~\ref{fig:meas-canc-no-circ} shows the measured amplitude and phased of the implemented conventional RF canceller without the antenna interface. The RF canceller has an amplitude tuning range between $-\SI{48}{dB}$ and $-\SI{17}{dB}$.

%%
\begin{figure}[t]
\centering
\subfloat{
\label{fig:meas-canc-no-circ-amp}
\includegraphics[width=0.8\columnwidth]{figs/meas/meas_canc_tx_rx_no_circ_amp.eps}} \\
\subfloat{
\label{fig:meas-canc-no-circ-phase}
\includegraphics[width=0.8\columnwidth]{figs/meas/meas_canc_tx_rx_no_circ_phase.eps}}
\vspace{-0\baselineskip}
\caption{Measured amplitude and phase of the implemented conventional RF canceller with (a) different attenuation codes, and (b) different phase shift codes.}
\label{fig:meas-canc-no-circ}
\vspace{-\baselineskip}
\end{figure}
%%

%%
\subsection{The Antenna Tuner}
In order to better match with the antenna interface, we also designed and implemented a programmable antenna tuner, which is used to match with varying impedance of the antenna due to environmental changes around $\SI{900}{MHz}$ operating frequency. In particular, a $\pi$-network with lossless inductor ($L$) and digitally tunable capacitors ($C_i$) are used for impedance transformation. In our implementation, we use a $\SI{5.1}{nH}$ chip inductor and the Peregrine $5$-bit PE64909 digitally tunable capacitors for $C_i$ ($i=1,2,3$). By programming the capacitors with codes \texttt{CAPi} ($i=1,2,3$), different antenna interface impedance matching can be achieved. The corresponding tuning range of the tunable capacitors is
%%
\begin{align*}
\texttt{CAPi} \in \{0,1,\cdots,31\},\ \forall i = 1,2,3.
\end{align*}
%%

%%
\begin{figure}[t]
\centering
\subfloat{
\label{fig:tuner-diagram}
\includegraphics[width=0.48\columnwidth]{figs/tuner_diagram.png}}
\subfloat{
\label{fig:tuner-pcb}
\includegraphics[width=0.48\columnwidth]{figs/tuner_pcb.png}}
\vspace{-0\baselineskip}
\caption{Diagram and PCB implementation of the programmable antenna tuner board.}
\label{fig:tuner}
\vspace{-\baselineskip}
\end{figure}
%%



%%
\subsection{Integration with the ORBIT Testbed}

Fig.~\ref{fig:canc-orbit-node} depicts the an FD ORBIT node equipped with the implemented conventional RF canceler. The node used is \texttt{node11-10} in the ORBIT \texttt{grid} with a USRP N210. In particular, the RF canceller TX/RX ports are connected to the USRP TX/RX ports, respectively, and the RF canceller CIRC port is connected to an Apex II-Multi-Band Antenna. 

%%
\begin{figure}[t]
\centering
\subfloat{
\label{fig:meas-canc}
\includegraphics[width=0.8\columnwidth]{figs/meas/meas_canc_orbit_onsite.eps}}
\vspace{-0\baselineskip}
\caption{Measured TX/RX isolation with and without using the conventional RF canceller. The $\SI{40}{dB}$ RF SIC bandwidth is $\SI{5}{MHz}$.}
\label{fig:meas-canc}
\vspace{-\baselineskip}
\end{figure}
%%

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_orbit"
%%% End:


==> tex/manual.tex <==

In this section, we provide a detailed guidance on how to use the FD ORBIT node. To facilitate experiments, a customized OS image named \mytexttt{flexicon-orbit-v1.ndz} has been created.


The simple FD transceiver example consists of two parallel programs (see Fig.~\ref{fig:diagram-orbit-node}). The first is an \mytexttt{UHD program} that is modified and extended based on the \mytexttt{tx\_waveforms} UHD example, where the TX and RX streaming sessions are running in parallel on the same carrier frequency in two separate threads. A third thread is also present for performing digital SIC. Pre-allocated global buffers are used to allow variables/buffers sharing between threads. The second is a \mytexttt{SUB20 program} used for controlling and configuring the SUB-20 controller.

\mytexttt{uhd\_find\_devices} can be used to check the configuration of the interface between the USRP N210 and \mytexttt{node11-10}.
The following commands can be used to execute the UHD program and configure the RF canceller:
\begin{lstlisting}[basicstyle=\ttfamily\small,language=c++]
$ ./fd_transceiver_simple -args
$ ./rf_canc_gen1_config -args
\end{lstlisting}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_orbit"
%%% End:

